Movable Antenna Optimization for Multi-User MIMO Systems in Realistic Ray-Traced Propagation Environments

To meet the growing data traffic demand in future wireless systems, novel transmission architectures capable of adapting to complex propagation environments are required. Movable antenna (MA) systems have recently emerged as a promising approach, enabling the physical repositioning of antenna elements to exploit spatial degrees of freedom. However, existing studies largely rely on idealized or simplistic channel models, leaving open the question of whether the performance gains of MA systems persist under realistic propagation conditions. This paper investigates the performance of downlink multi-user MIMO systems with movable antennas using deterministic ray-traced channel models. A simulation framework combining three-dimensional ray tracing and field-response channel modeling is developed, and antenna positions are optimized using particle swarm optimization and genetic algorithms. Simulation results reveal that while simplified distance-based channel models predict large performance disparities between competing array configurations, realistic ray-traced channels significantly compress these differences, indicating that propagation effects dominate over pure array geometry optimization. Nevertheless, movable antenna systems retain strong effectiveness over conventional fixed arrays across different user distributions, array sizes, and multipath conditions, even in geometry-constrained propagation environments.

==> macro.TeX <==


    %\newcommand{\tr}{\mbox{trace}}
    \def\bm#1{\boldsymbol{#1}}
    \def\ang#1{\mbox{$\langle #1 \rangle$}}
    \def\aang#1{\mbox{$\langle\!\langle #1 \rangle\!\rangle$}}

    \def\mnorm#1{\mbox{$\left|\!\left|\!\left|\, #1 \,\right|\!\right|\!\right|$}}



    \def\Complex{{\rm\rule[.23ex]{.03em}{1.1ex}\kern-.3em{C}}}
    \def\bms#1{\mbox{\boldmath $\scriptstyle #1$}}
    \def\eqover#1{\mbox{$\buildrel #1 \over =$}}
    \def\leqover#1{\mbox{$\buildrel #1 \over \leq$}}
    \def\Imag#1{\mbox{${\Im}\left\{ #1 \right\}$}}
    \def\dist{\mbox{${\sf dist}(z, {\mathbb R}^+)$}}
    \def\largeN{\mbox{${\cal N}$}}

    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof: }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof: }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  %\newtheorem{theorem}{Theorem}
  %\newtheorem{conjecture}{Conjecture}
  %\newtheorem{definition}{Definition}
  %\newtheorem{example}{Example}
  %\newtheorem{lemma}{Lemma}
  %\newtheorem{proposition}{Proposition}
  %\newtheorem{claim}{Claim}

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

    %%%%%% DEFINITION %%%%%%%%%%%%%%
    \newcommand{\qa}{{\bf a}}
        \newcommand{\qb}{{\bf b}}
        \newcommand{\qc}{{\bf c}}
        \newcommand{\qd}{{\bf d}}
        \newcommand{\qe}{{\bf e}}
        \newcommand{\qf}{{\bf f}}
        \newcommand{\qg}{{\bf g}}
        \newcommand{\qh}{{\bf h}}
        \newcommand{\qi}{{\bf i}}
        \newcommand{\qj}{{\bf j}}
        \newcommand{\qk}{{\bf k}}
        \newcommand{\ql}{{\bf l}}
        \newcommand{\qm}{{\bf m}}
        \newcommand{\qn}{{\bf n}}
        \newcommand{\qo}{{\bf o}}
        \newcommand{\qp}{{\bf p}}
        \newcommand{\qq}{{\bf q}}
        \newcommand{\qr}{{\bf r}}
        \newcommand{\qs}{{\bf s}}
        \newcommand{\qt}{{\bf t}}
        \newcommand{\qu}{{\bf u}}
        \newcommand{\qv}{{\bf v}}
        \newcommand{\qw}{{\bf w}}
        \newcommand{\qx}{{\bf x}}
        \newcommand{\qy}{{\bf y}}
        \newcommand{\qz}{{\bf z}}
    
        \newcommand{\qA}{{\bf A}}
        \newcommand{\qB}{{\bf B}}
        \newcommand{\qC}{{\bf C}}
        \newcommand{\qD}{{\bf D}}
        \newcommand{\qE}{{\bf E}}
        \newcommand{\qF}{{\bf F}}
        \newcommand{\qG}{{\bf G}}
        \newcommand{\qH}{{\bf H}}
        \newcommand{\qI}{{\bf I}}
        \newcommand{\qJ}{{\bf J}}
        \newcommand{\qK}{{\bf K}}
        \newcommand{\qL}{{\bf L}}
        \newcommand{\qM}{{\bf M}}
        \newcommand{\qN}{{\bf N}}
        \newcommand{\qO}{{\bf O}}
        \newcommand{\qP}{{\bf P}}
        \newcommand{\qQ}{{\bf Q}}
        \newcommand{\qR}{{\bf R}}
        \newcommand{\qS}{{\bf S}}
        \newcommand{\qT}{{\bf T}}
        \newcommand{\qU}{{\bf U}}
        \newcommand{\qV}{{\bf V}}
        \newcommand{\qW}{{\bf W}}
        \newcommand{\qX}{{\bf X}}
        \newcommand{\qY}{{\bf Y}}
        \newcommand{\qZ}{{\bf Z}}
        \newcommand{\qzero}{{\bf 0}}
        \newcommand{\qone}{{\bf 1}}
        \newcommand{\qdh}{\triangle\qh}
        \newcommand{\qhh}{\hat\qh}
        \newcommand{\qdH}{\triangle\qH}
        \newcommand{\qhH}{\hat\qH}
        \newcommand{\qdF}{\triangle\qF}
        \newcommand{\qhF}{\hat\qF}
        \newcommand{\qbh}{\bar\qh}
        \newcommand{\qbn}{\bar\qn}
        \newcommand{\quH}{\underline{\qH}}
        \newcommand{\quh}{\underline{\qh}}
        \newcommand{\uh}{\underline{h}}
        \newcommand{\quY}{\underline{\qY}}
        \newcommand{\quy}{\underline{\qy}}
        \newcommand{\uy}{\underline{y}}
        \newcommand{\quZ}{\underline{\qZ}}
        \newcommand{\quz}{\underline{\qz}}
        \newcommand{\uz}{\underline{z}}
    
    
    
    
    
    
        \newcommand{\qwbE}{\overline{\bf E}}
        \newcommand{\qwbF}{\overline{\bf F}}
        \newcommand{\qwbT}{\overline{\bf T}}
        \newcommand{\qwbR}{\overline{\bf R}}
    
        \newcommand{\qDelta}{{\boldsymbol \Delta}}
        \newcommand{\qPsi}{{\boldsymbol \Psi}}
        \newcommand{\qPhi}{{\boldsymbol \Phi}}
        \newcommand{\qXi}{{\boldsymbol \Xi}}
        \newcommand{\qTheta}{{\boldsymbol \Theta}}
        \newcommand{\qLambda}{{\boldsymbol \Lambda}}
        \newcommand{\qSigma}{{\boldsymbol \Sigma}}
        \newcommand{\qGamma}{{\boldsymbol \Gamma}}
        \newcommand{\qUpsilon}{{\boldsymbol \Upsilon}}
        \newcommand{\qOmega}{{\boldsymbol \Omega}}
        \newcommand{\qPi}{{\boldsymbol \Pi}}
    
        \newcommand{\qalpha}{{\boldsymbol \alpha}}
        \newcommand{\qbeta}{{\boldsymbol \beta}}
        \newcommand{\qdelta}{{\boldsymbol \delta}}
        \newcommand{\qlambda}{{\boldsymbol \lambda}}
        \newcommand{\qgamma}{{\boldsymbol \gamma}}
        \newcommand{\qepsilon}{{\boldsymbol \epsilon}}
        \newcommand{\qeta}{{\boldsymbol \eta}}
        \newcommand{\qnu}{{\boldsymbol \nu}}
        \newcommand{\qmu}{{\boldsymbol \mu}}
        \newcommand{\qkappa}{{\boldsymbol \kappa}}
        \newcommand{\qtau}{{\boldsymbol \tau}}
        \newcommand{\qxi}{{\boldsymbol \xi}}
        \newcommand{\qzeta}{{\boldsymbol \zeta}}
        \newcommand{\qvarepsilon}{{\boldsymbol \varepsilon}}
        \newcommand{\qomega}{{\boldsymbol \omega}}
        \newcommand{\qsigma}{{\boldsymbol \sigma}}
        \newcommand{\qrho}{{\boldsymbol \rho}}
        \newcommand{\qtheta}{{\boldsymbol \theta}}
    
    
        \newcommand{\tH}{{\tilde{H}}}
        \newcommand{\talpha}{{\tilde{\alpha}}}
        \newcommand{\ttau}{{\tilde{\tau}}}
        \newcommand{\te}{{\tilde{e}}}
        \newcommand{\tb}{{\tilde{b}}}
        \newcommand{\tv}{{\tilde{v}}}
        \newcommand{\trho}{{\tilde{\rho}}}
        \newcommand{\tvarepsilon}{{\tilde{\varepsilon}}}
    
        \newcommand{\tqH}{{\tilde{\qH}}}
        \newcommand{\tqU}{{\tilde{\qU}}}
        \newcommand{\tqD}{{\tilde{\qD}}}
        \newcommand{\tqQ}{{\tilde{\qQ}}}
        \newcommand{\tqTheta}{{\tilde{\qTheta}}}
        \newcommand{\tqDelta}{{\tilde{\qDelta}}}
        \newcommand{\tqPsi}{{\tilde{\qPsi}}}
        \newcommand{\tqPhi}{{\tilde{\qPhi}}}
        \newcommand{\tcalqS}{{\tilde{\calqS}}}
        \newcommand{\tqXi}{{\tilde{\qXi}}}
        \newcommand{\tqv}{{\tilde{\qv}}}
        \newcommand{\tqLambda}{{\tilde{\qLambda}}}
    
        \newcommand{\bH}{{\bar{H}}}
        \newcommand{\bqH}{{\bar{\qH}}}
    
        \newcommand{\uqB}{{\underline{\qB}}}
        \newcommand{\uH}{{\underline{H}}}
        \newcommand{\utH}{{\underline{\tH}}}
        \newcommand{\ubH}{{\underline{\bH}}}
        \newcommand{\uR}{{\underline{R}}}
        \newcommand{\uT}{{\underline{T}}}
        \newcommand{\uqH}{{\underline{\qH}}}
        \newcommand{\uqR}{{\underline{\qR}}}
        \newcommand{\uqT}{{\underline{\qT}}}
        \newcommand{\ubqH}{{\underline{\bqH}}}
        \newcommand{\utqH}{{\underline{\tqH}}}
        \newcommand{\ucalqX}{{\underline{\calqX}}}
        \newcommand{\uqX}{{\underline{\qX}}}
    
        \newcommand{\bbB}{{\mathbb B}}
        \newcommand{\bbE}{{\mathbb E}}
        \newcommand{\bbN}{{\mathbb N}}
        \newcommand{\bbR}{{\mathbb R}}
        \newcommand{\bbC}{{\mathbb C}}
        \newcommand{\bbS}{{\mathbb S}}
        \newcommand{\bbU}{{\mathbb U}}
        \newcommand{\bbQ}{{\mathbb Q}}
    
        \newcommand{\calA}{{\mathcal A}}
        \newcommand{\calB}{{\mathcal B}}
        \newcommand{\calC}{{\mathcal C}}
        \newcommand{\calD}{{\mathcal D}}
        \newcommand{\calE}{{\mathcal E}}
        \newcommand{\calF}{{\mathcal F}}
        \newcommand{\calI}{{\mathcal I}}
        \newcommand{\calK}{{\mathcal K}}
        \newcommand{\calL}{{\mathcal L}}
        \newcommand{\calN}{{\mathcal N}}
        \newcommand{\calO}{{\mathcal O}}
        \newcommand{\calP}{{\mathcal P}}
        \newcommand{\calQ}{{\mathcal Q}}
        \newcommand{\calS}{{\mathcal S}}
        \newcommand{\calV}{{\mathcal V}}
        \newcommand{\calX}{{\mathcal X}}
        \newcommand{\calCN}{{\mathcal{N}_{\mathbb C}}}
    
    
    
        \newcommand{\calqB}{\boldsymbol{\cal B}}
        \newcommand{\calqX}{\boldsymbol{\cal X}}
        \newcommand{\calqS}{\boldsymbol{\cal S}}
    
        \newcommand{\dom}{{\sf dom}}
        \newcommand{\epi}{{\sf epi}}
        \newcommand{\diag}{{\sf diag}}
        \newcommand{\supp}{{\sf supp}}
        \newcommand{\tr}{{\sf tr}}
        \newcommand{\Ex}{{\sf E}}
        \newcommand{\rank}{{\sf rank}}
        \newcommand{\Varx}{{\sf Var}}
    
        \newcommand*{\argmin}{\operatornamewithlimits{argmin}\limits}
        \newcommand*{\argmax}{\operatornamewithlimits{argmax}\limits}
    
        \newcommand{\sfj}{{\sf j}}
    
        \newcommand{\sfC}{{\sf C}}
        \newcommand{\sfF}{{\sf F}}
        \newcommand{\sfX}{{\sf X}}
        \newcommand{\sfZ}{{\sf Z}}
        \newcommand{\sfqB}{\boldsymbol{\sf B}}
        \newcommand{\sfqX}{\boldsymbol{\sf X}}
        \newcommand{\sfqx}{\boldsymbol{\sf x}}
    
    
    
    
    
    
        \newcommand{\aaa}{\buildrel{\circ}\over{a}}
        \newcommand{\aeta}{\buildrel{\circ}\over{\eta}}
        \newcommand{\arho}{\buildrel{\circ}\over{\rho}}
        \newcommand{\aalpha}{\buildrel{\circ}\over{\alpha}}
        \newcommand{\ateta}{\buildrel{\circ}\over{\tilde\eta}}
        \newcommand{\atalpha}{\buildrel{\circ}\over{\tilde\alpha}}
        \newcommand{\atrho}{\buildrel{\circ}\over{\tilde\rho}}
    
    
        \newcommand{\bfbl}[1]{\bf \color{blue}#1}
        \newcommand{\bl}[1]{\color{blue}#1}
        \newcommand{\bfrl}[1]{\bf \color{red}#1}
        \newcommand{\rl}[1]{\color{red}#1}
        \newcommand{\bfbrl}[1]{\bf \color{BrickRed}#1}
        \newcommand{\bfbbl}[1]{\bf \color{BlueViolet}#1}




    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

